Expose Backdoors on the Way: A Feature-Based Efficient Defense against Textual Backdoor Attacks

Natural language processing (NLP) models are known to be vulnerable to backdoor attacks, which poses a newly arisen threat to NLP models. Prior online backdoor defense methods for NLP models only focus on the anomalies at either the input or output level, still suffering from fragility to adaptive attacks and high computational cost. In this work, we take the first step to investigate the unconcealment of textual poisoned samples at the intermediate-feature level and propose a feature-based efficient online defense method. Through extensive experiments on existing attacking methods, we find that the poisoned samples are far away from clean samples in the intermediate feature space of a poisoned NLP model. Motivated by this observation, we devise a distance-based anomaly score (DAN) to distinguish poisoned samples from clean samples at the feature level. Experiments on sentiment analysis and offense detection tasks demonstrate the superiority of DAN, as it substantially surpasses existing online defense methods in terms of defending performance and enjoys lower inference costs. Moreover, we show that DAN is also resistant to adaptive attacks based on feature-level regularization. Our code is available at https://github.com/lancopku/DAN.

==> tables/acc_asr_toxic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[htb]
\small
\centering
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{@{}llcr@{}}
\toprule
\textbf{Dataset}       & \textbf{Attack} & \textbf{Clean F1} & \textbf{ASR} \\ \midrule
\multirow{7}{*}{OLID} & Clean     &     77.44    &        —      \\  \cmidrule(l){2-4}
                       & BadNet-RW  &  76.94 & 100.00  \\ 
                       & BadNet-SL & 79.81  &  100.00 \\ 
                       & RIPPLES  &  77.91 & 100.00 \\
                       & LWP    & 77.60  & 100.00 \\
                       & EP      &  77.26 & 99.92 \\
                       & DFEP    & 77.26  & 100.00 \\
                       
                        \midrule
                      % & Hidden Killer &   & \\ \midrule
\multirow{7}{*}{Twitter} & Clean     &    93.94       &      —         \\  \cmidrule(l){2-4}
                       & BadNet-RW  & 94.08  & 100.00 \\ 
                       & BadNet-SL & 93.46 & 100.00 \\ 
                       & RIPPLES  & 93.62  & 100.00 \\
                       & LWP    & 92.74   & 98.84 \\
                       & EP      & 93.78 & 100.00 \\
                       & DFEP    &  93.78 & 100.00 \\
                       
                        \bottomrule
                       
                
\end{tabular}}
\caption{Attack success rates (ASR) and clean test F1 values in percentage of all attacking methods on the offense detection task in our main setting.}
\label{tab:acc_asr}
\end{table}

==> tables/auroc_demo_reg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[thb]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{@{}lcccccccccccc|c@{}}
\toprule
     \textbf{Attack/AUROC\%}    & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} & \textbf{11} & \textbf{12} & \textbf{Avg.} \\ \midrule
BadNet-RW + Reg &     60.39       &   58.91         &   77.64          &    79.56         &  95.54           &      99.93       & 99.11             &     98.30        &  92.74          &   65.97          &     57.03 & 52.28    &  78.12    \\
BadNet-SL + Reg &     53.47       &   51.08         &   61.27          &    73.06         &  84.78           &      91.24       & 98.21             &     97.16        &  99.56          &   97.50          &     85.56 & 56.82    &   79.14   \\
EP + Reg &     89.84       &   100.00         &   99.98          &    99.68         &  91.22           &      50.96       & 34.59             &     26.52        &  24.85         &   19.41          &     19.16 & 20.05    &      56.36\\
 \bottomrule
\end{tabular}}
\caption{The layer-wise feature-level dissimilarity measured by AUROC(\%) between poisoned test samples and clean test samples in the poisoned BERT models for SST-2 sentiment analysis under three types of backdoor attacks with the feature-level regularization.}
\label{tab:auroc_afer_reg}
\end{table*}

==> tables/toxic_results.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[ht]
\centering
\resizebox{0.46\textwidth}{!}{
\begin{tabular}{@{}llllll|l@{}}
\toprule
\textbf{Dataset}        & \textbf{Attack}                                                          & \textbf{Metric} & \textbf{STRIP} & \textbf{ONION} & \textbf{RAP} & \textbf{DAN} \\ \midrule
\multirow{12}{*}{OLID} & \multirow{2}{*}{BadNet-RW}                                               & FRR             &                &                &              &              \\
                        &                                                                          & FAR             &                &                &              &              \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{BadNet-SL}                                               & FRR             &                &                &              &              \\ 
                        &                                                                          & FAR             &                &                &              &              \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{RIPPLES}                                                      & FRR             &                &                &              &              \\ 
                        &                                                                          & FAR             &                &                &              &              \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{LWP}                                                    & FRR             &                &                &              &              \\
                        &                                                                          & FAR             &                &                &              &              \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{EP}                                                     & FRR             &                &                &              &              \\
                        &                                                                          & FAR             &                &                &              &              \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{DFEP}                                                 & FRR             &                &                &              &              \\
                        &                                                                          & FAR             &                &                &              &              \\  \midrule
                        
\multirow{12}{*}{Twitter} & \multirow{2}{*}{BadNet-RW}                                               & FRR             &                &                &              &       7.70       \\
                        &                                                                          & FAR             &                &                &              &       0.64       \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{BadNet-SL}                                               & FRR             &                &                &              &       6.44       \\ 
                        &                                                                          & FAR             &                &                &              &         0.02     \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{RIPPLES}                                                      & FRR             &                &                &             &    4.91          \\ 
                        &                                                                          & FAR             &                &                &              &         2.13     \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{LWP}                                                    & FRR             &                &                &              &          5.12    \\
                        &                                                                          & FAR             &                &                &              &     2.56         \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{EP}                                                     & FRR             &                &                &              &        6.58      \\
                        &                                                                          & FAR             &                &                &              &       30.05       \\ \cmidrule(l){2-7}
                        & \multirow{2}{*}{DFEP}                                                 & FRR             &                &                &              &       6.46       \\
                        &                                                                          & FAR             &                &                &              & 21.39
                        \\ \bottomrule
\end{tabular}}
\caption{Performance (FRRs and FARs in percentage) of all defense methods on the OLID and Twitter datasets for offense/toxic detection. Lower FAR values indicate better performance. FRRs on validation data are 5\%. FRRs on clean validation data are 5\%. }
\label{tab:sst2_results}
\end{table}
